Doomsday Equilibria for Omega-Regular Games

Two-player games on graphs provide the theoretical frame- work for many important problems such as reactive synthesis. While the traditional study of two-player zero-sum games has been extended to multi-player games with several notions of equilibria, they are decidable only for perfect-information games, whereas several applications require imperfect-information games. In this paper we propose a new notion of equilibria, called doomsday equilibria, which is a strategy profile such that all players satisfy their own objective, and if any coalition of players deviates and violates even one of the players objective, then the objective of every player is violated. We present algorithms and complexity results for deciding the existence of doomsday equilibria for various classes of omega-regular objectives, both for imperfect-information games, and for perfect-information games. We provide optimal complexity bounds for imperfect-information games, and in most cases for perfect-information games.

==> preliminaries.tex <==
\section{Game Arena with Perfect Information and Very Nice Equilibria}\label{sec:prelim}

\paragraph{{\bf Game Arena}} 
%
An $n$-player game arena $G$ (with perfect information) is a tuple $(S, {\cal P},s_{{\sf init}}, \Sigma, \Delta)$ such that 
\begin{itemize}
	\item $S$ is a nonempty finite set of \textit{states} and ${\cal P}=\{S_1,S_2,\dots,S_n\}$ is a partition of $S$ into $n$ classes of states, one for each Player~$i \in \{ 1,2,\dots,n\}$, 
	\item $s_{{\sf init}} \in S$ is the initial state, 
	\item $\Sigma$ is set of a finite alphabet,  
	\item and $\Delta : S \times \Sigma \rightarrow S$ is the transition function of the game.
\end{itemize}
%
Plays in $n$-player game arena $G$ are constructed as follows. They start in the initial state $s_{{\sf init}}$, and then a $\omega$ number of rounds are played as follows: the player that owns the current state $s$ choose a letter $\sigma \in \Sigma$ and the game evolves to the position defined by $\Delta(s,\sigma)$, then a new round is started from there. So, more formally, a {\em play} in $G$ is an infinite sequence $s_0 s_1 \dots s_n \dots$ such that $(i)$ $s_0=s_{{\sf init}}$ and $(i)$ for all $i \geq 0$, there exists $\sigma \in \Sigma$ such that $s_{i+1}=\Delta(s_i,\sigma)$. 
%
The set of plays in $G$ is noted by $\plays(G)$, and the set of prefixes of plays by $\prefplays(G)$. We denote by $\rho,\rho_1,\rho_i, \dots$ plays in $G$, by $\rho(0..j)$ the prefix of the play $\rho$ up to position $j$ and by $\rho(j)$ the position $j$ in the play $\rho$. We also use $\pi$, $\pi_1$, $\pi_2$, ... to denote prefixes of plays. Let $i \in \{1,2,\dots,n\}$, a prefix $\pi$ belongs to Player~$i$ if ${\sf last}(\pi)$, the last state of $\pi$, belongs to Player~$i$, i.e. ${\sf last}(\pi) \in S_i$. We denote by $\prefplays_i(G)$ the set of prefixes in $G$ that belongs to Player~$i$.


\paragraph{{\bf Strategies and strategy profiles}} 
%
Strategies are defined as usual as mappings from prefixes of plays to actions. 
A {\em strategy} for Player~$i$, $i \in \{1,2,\dots,n\}$, is a function $\lambda_i :  \prefplays_i(G) \rightarrow \Sigma$.
%
A {\em strategy profile} $\Lambda = (\lambda_1,\lambda_2,\dots,\lambda_n)$ is a tuple of strategies such that
$\lambda_i$ is a strategy of Player $i$. Given a strategy profile $\Lambda= (\lambda_1,\lambda_2,\dots,\lambda_n)$, we also denote the strategy $\lambda_i$ by $\Lambda_i$ and the the tuple of the remaining strategies $(\lambda_1,\dots,\lambda_{i-1},\lambda_{i+1},\dots,\lambda_n)$ by  $\Lambda_{-i}$. 
%
For a strategy $\lambda_i$ of Player $i$, we define its {\em outcome} as the set of plays that are consistent with $\lambda_i$: formally, 
$\outcome_i(\lambda_i)$ is the set of $\rho \in \plays(G)$ such that for all $j \geq 0$, if $\rho(0..j) \in \prefplays_i(G)$, then $\rho(j+1)=\Delta(\rho(j),\lambda_i(\rho(0..j)))$.
%
Similarly, we define the {\em outcome of a strategy profile} $\Lambda=(\lambda_1,\lambda_2,\dots,\lambda_n)$, as the unique play $\rho \in \plays(G)$ such that for all positions $j$, for all $i \in \{1,2,\dots,n\}$, if $\rho(j) \in \prefplays_i(G)$ then $\rho(j+1)=\Delta(\rho(j),\lambda_i(\rho(0..j)))$.
%
Clearly, we have that $\outcome(\Lambda)=\bigcap_{1 \leq i \leq n} \outcome_i(\lambda_i)$.




\paragraph{{\bf Winning conditions}}
A {\em winning condition} $W_i$ for Player $i \in \{1,2,\dots,n\}$ is a set of set of infinite sequence of states, i.e. $W_i \subseteq S^{\omega}$. 
%
A strategy $\lambda_i$ is {\em winning} for Player $i$ (against all other players) w.r.t. a winning condition $W_i$ if
$\outcome_i(\lambda_i)\subseteq W_i$. 

%\marginpar{{\bf JF}: Do we need to introduce the notion of Nash equilibrium here ?}
%For a tuple of winning conditions $\overline{\phi} =
%(\phi_1,\dots,\phi_n)$, and a strategy profile $\overline{\sigma}$,
%the value of $\overline{\sigma}$, denoted by
%$v_{\overline{\phi}}(\overline{\sigma})$, is an $n$-tuple in
%$\{0,1\}^n$ defined by $(v_{\overline{\phi}}(\overline{\sigma}))_i =
%1$ iff $\overline{\sigma}_i$ is winning for Player $i$ wrt $\phi_i$.
%
%
%\paragraph{Nash Equilibria} A strategy profile $\overline{\sigma} = (\sigma_1,\dots,\sigma_n)$ is
%a \textit{Nash Equilibrium} if for all $i\in\{1,\dots,n\}$, for all
%strategy $\lambda_i$ of Player $i$:
%$$
%(v_{\overline{\phi}}(\sigma_1,\dots,\sigma_{i-1},\sigma_{i},\sigma_{i+1},\dots,\sigma_n))_i \geq (v_{\overline{\phi}}(\sigma_1,\dots,\sigma_{i-1},\lambda_i,\sigma_{i+1},\dots,\sigma_n))_i
%$$


%
Given $n$ winning conditions $W_1,\dots,W_n$, one for each Player~$i$, $i \in \{1,2,\dots,n\}$, a strategy profile
$\Lambda=(\lambda_1,\lambda_2,\dots,\lambda_n)$ is {\em winning} if $\outcome(\Lambda) \in \bigcap_i W_i$.
Given an infinite sequence of states $\rho \in S^{\omega}$, we note ${\sf visit}(\rho)$ the set of states that appears at least once along $\rho$, i.e. ${\sf visit}(\rho)=\{ s \in S | \exists i \geq 0 \rho(i)=s \}$, and ${\sf inf}(\rho)$ the set of states that appears infinitely often along $\rho$, i.e. ${\sf inf}(\rho)=\{ s \in S | \forall i \geq \cdot \exists j \geq i \cdot \rho(i)=s \}$.

We consider the following types of winning conditions:
  \begin{itemize}
  	\item a {\em safety objective} is defined by a subset of states $T \subseteq S$ that should not be left: ${\sf safe}(T)=\{ \rho \in S^{\omega} \mid {\sf visit}(\rho) \subseteq T \}$;  
  	\item a {\em reachability objective} is defined by a subset of states $T \subseteq S$ that has to be reached: ${\sf reach}(T)=\{ \rho \in S^{\omega} \mid {\sf visit}(\rho) \cap T \not= \emptyset \}$; 
	\item a {\em Buchi objective} is defined by a subset of states $T \subseteq S$ that has to be visited infinitely often: ${\sf Buchi}(T)=\{ \rho \in S^{\omega} \mid {\sf inf}(\rho) \cap T \not= \emptyset \}$; 
	\item a {\em co-Buchi objective} is defined by a subset of states $T \subseteq S$ that has to be reached eventually and never left: ${\sf co-Buchi}(T)=\{ \rho \in S^{\omega} \mid {\sf inf}(\rho) \subseteq T \}$; 
	\item let $d \in \nat$, a {\em parity objective with $d$ priorities} is a condition which is defined with a parity function $p : S \rightarrow  \{0,1,\dots,d\}$ such that the minimal priority among the set of states that are visited infinitely often is even: ${\sf parity}(p)=\{ \rho \in S^{\omega} | \min \{ p(s) \mid s \in {\sf inf}(\rho)\} \mbox{~is~even} \}$.
  \end{itemize}
B\"uchi, co-B\"uchi and parity objectives are called {\em tail objectives} because they enjoy the following closure property: Let $W$ be a B\"uchi, co-B\"uchi and parity objective, for all $\rho \in W$ and for all $\pi \in S^{*}$, we have that $\pi \cdot \rho \in W$.

\paragraph{{\bf Very Nice Equilibrium}} A strategy profile $\Lambda=(\lambda_1,\lambda_2,\dots,\lambda_n)$ is a 
{\em very nice equilibrium} if:
\begin{enumerate}
  \item $(1)$ it is winning for all the players, i.e. for all $\rho\in
    \outcome(\Lambda)$, $\rho\in\bigcap_i W_i$;

  \item $(2)$ and all players are able to retaliate in case of deviation: for all $i$, $1 \leq i \leq n$, for all $\rho\in \outcome_i(\lambda_i)$, if
    $\rho\not\in W_i$, then $\rho \in \bigcap_{i\neq j} \overline{W_j}$. 

\end{enumerate}

In other words, when all the players stick to their strategies then they all win, and if some player deviates and causes another player to lose then this player can retaliate and make all other players lose. 

\paragraph{Relation with Secure Equilibria}
The two-player case of our notion of very nice equilibrium coincides with the notion of secure equilibrium defined in~\cite{}.


%% \paragraph{Remark} We could also require that at least one of the
%% Player can punish any selfish Player:

%% \begin{enumerate}
%%   \item[4.] \textbf{there exists} $i$, $\outcome(\lambda_i)\models (\bigvee_{i\neq
%%     j} W_j)\rightarrow W_i$. 
%% \end{enumerate}


\paragraph{{\bf Example}} 
Insert here a small example (game arena+safety+explain the main ingredients).
%Consider the following specification of a mutual
%exclusion protocol:
%$$
%\bigwedge_{i=1}^n (\always \eventually a_i)\wedge \always
%(a_i\rightarrow \bigwedge_{j\neq i} \neg a_j)
%$$
%
%A very nice equilibrium for this spec is defined by the strategies
%$\lambda_i$ which count up to $n$ and hold the token
%at rank $i$ and releases it at rank $i+1$. If some player has changed his strategy, it may create
%a conflict. To punish all the other players you just have to hold the
%token all the time after you got the first conflict.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

